Ratio of $\bar{\Lambda}$ to $K_\rm{S}^0$ production cross-sections in $pp$ collisions at 13.6TeV

The production cross-section ratio of promptly produced $\bar{\Lambda}$ and $K_\rm{S}^0$ hadrons is measured in proton-proton collision data at a centre-of-mass energy of 13.6TeV recorded in 2024 with the upgraded LHCb detector and corresponding to an integrated luminosity of $64\rm{pb}^{-1}$. The ratio is presented as a function of transverse momentum, $p_\rm{T}$, and rapidity, $y$, in the ranges $0.15 < p_\rm{T} < 2.5\rm{GeV}/c$ and $2.0 < y < 4.5$. The results are in good agreement with previous measurements at different centre-of-mass energies. They are compared to predictions from currently available event generators and can be used as input in future event generator tunings.

==> Authorship_LHCb-PAPER-2026-045-arXiv.tex <==
LHCb collaboration:
R. Aaij,
M. Abdelfatah,
A.S.W. Abdelmotteleb,
C. Abellan Beteta,
F. Abudin\'en,
T. Ackernley,
A.A. Adefisoye,
B. Adeva,
M. Adinolfi,
P. Adlarson,
C. Agapopoulou,
L. Ahrens,
C.A. Aidala,
S. Akar,
K. Akiba,
H. Al Saleh,
P. Albicocco,
J. Albrecht,
R. Aleksiejunas,
F. Alessio,
P. Alvarez Cartelle,
A.A. Alves Jr,
S. Amato,
Y. Amhis,
Z. Amos,
L. An,
L. Anderlini,
P. Andreola,
M. Andreotti,
S. Andres Estrada,
A. Anelli,
C. Arata,
F. Archilli,
Z. Areg,
M. Argenton,
S. Arguedas Cuendis,
L. Arnone,
M. Artuso,
E. Aslanides,
R. Ata\'ide Da Silva,
M. Atzeni,
B. Audurier,
J.A. Authier,
D. Bacher,
I. Bachiller Perea,
S. Bachmann,
J.J. Back,
M. Bai,
Z.B. Bai,
V. Balagura,
A. Balboni,
W. Baldini,
L. Balzani,
H. Bao,
J. Baptista de Souza Leite,
C. Barbero Pretel,
I.R. Barbosa,
W. Barker,
R.J. Barlow,
M. Barnyakov,
S. Baron,
S. Barsuk,
W. Barter,
J. Bartz,
S. Bashir,
B. Batsukh,
P.B. Battista,
A. Bavarchee,
A. Bay,
A. Beck,
M. Becker,
F. Bedeschi,
I.B. Bediaga,
N.A. Behling,
S. Belin,
A. Bellavista,
I. Belyaev,
G. Bencivenni,
E. Ben-Haim,
J.L.M. Berkey,
R. Bernet,
A. Bertolin,
L. Bertsch,
F. Betti,
J. Bex,
O. Bezshyyko,
S. Bhattacharya,
M.S. Bieker,
N.V. Biesuz,
A. Biolchini,
M. Birch,
F.C.R. Bishop,
A. Bitadze,
A. Bizzeti,
F. Blanc,
J.E. Blank,
S. Blusk,
J.A. Boelhauve,
O. Boente Garcia,
T. Boettcher,
A. Bohare,
C. Bolognani,
R.B. Bonacci,
A. Bordelius,
F. Borgato,
S. Borghi,
M. Borsato,
J.T. Borsuk,
E. Bottalico,
M. Bovill,
T.J.V. Bowcock,
A. Boyer,
C. Bozzi,
J.D. Brandenburg,
A. Brea Rodriguez,
N. Breer,
C. Breitfeld,
J. Brodzicka,
J. Brown,
E. Buchanan,
M. Burgos Marcos,
C. Burr,
E. Butera,
C. Buti,
J.S. Butter,
W. Byczynski,
S. Cadeddu,
H. Cai,
Y. Cai,
Y. Cai,
A. Caillet,
R. Calabrese,
L. Calefice,
M. Calvi,
M. Calvo Gomez,
P. Camargo Magalhaes,
J.I. Cambon Bouzas,
P. Campana,
A. Campomagnani,
A.C. Campos,
A.F. Campoverde Quezada,
Y. Cao,
S. Capelli,
M. Caporale,
L. Capriotti,
R. Caravaca-Mora,
A. Carbone,
L. Carcedo Salgado,
R. Cardinale,
A. Cardini,
P. Carniti,
M. Carou Laino,
L. Carus,
R. Caspary,
G. Casse,
M. Cattaneo,
G. Cavallero,
V. Cavallini,
S. Celani,
I. Celestino,
S. Cesare,
A.J. Chadwick,
M. Charles,
Ph. Charpentier,
E. Chatzianagnostou,
R. Cheaib,
M. Chefdeville,
C. Chen,
J. Chen,
S. Chen,
Z. Chen,
A. Chen Hu,
M. Cherif,
S. Chernyshenko,
X. Chiotopoulos,
G. Chizhik,
V. Chobanova,
A. Christakakis,
M. Chrzaszcz,
Y. Chu,
V. Chulikov,
P. Ciambrone,
X. Cid Vidal,
P. Cifra,
P.E.L. Clarke,
M. Clemencic,
H.V. Cliff,
J. Closier,
C. Cocha Toapaxi,
V. Coco,
A. Codovini,
C.S. Codovini,
J. Cogan,
E. Cogneras,
L. Cojocariu,
S. Collaviti,
P. Collins,
T. Colombo,
M. Colonna,
A. Comerma-Montells,
L. Congedo,
J. Connaughton,
A. Contu,
N. Cooke,
A. Corallo,
G. Cordova,
C. Coronel,
I. Corredoira ,
A. Correia,
G. Corti,
G.C. Costantino,
C. Cotirlan,
J. Cottee Meldrum,
B. Couturier,
D.C. Craik,
N. Crepet,
M. Cruz Torres,
M. Cubero Campos,
E. Curras Rivera,
R. Currie,
C.L. Da Silva,
X. Dai,
J. Dalseno,
C. D'Ambrosio,
G. Darze,
A. Davidson,
O. De Aguiar Francisco,
C. De Angelis,
F. De Benedetti,
J. de Boer,
K. De Bruyn,
S. De Capua,
M. De Cian,
U. De Freitas Carneiro Da Graca,
F. De Gregorio,
E. De Lucia,
J.M. De Miranda,
L. De Paula,
A. De Robertis,
E. De Santis,
M. De Serio,
P. De Simone,
F. De Vellis,
J.A. de Vries,
F. Debernardis,
D. Decamp,
S. Dekkers,
L. Del Buono,
B. Demaire-Lepape,
J. Deng,
O. Deschamps,
F. Dettori,
B. Dey,
A. Di Canto,
P. Di Nezza,
S. Ding,
Y. Ding,
L. Dittmann,
J.F. Diverchy,
A.D. Docheva,
A. Doheny,
C. Dong,
F. Dordei,
J. Dorta Moreno,
A.C. dos Reis,
J. Dos Santos Oliveira,
A.D. Dowling,
L. Dreyfus,
W. Duan,
N. Duc,
P. Duda,
L. Dufour,
V. Duk,
P. Durante,
M.M. Duras,
J.M. Durham,
K. Duwe,
A. Dziurda,
S. Easo,
E. Eckstein,
U. Egede,
S. Eisenhardt,
E. Ejopu,
L. Eklund,
M. Elashri,
D. Elizondo Blanco,
J. Ellbracht,
S. Ely,
A. Ene,
T. Evans,
F. Fabiano,
S. Faghih,
L.N. Falcao,
B. Fang,
R. Fantechi,
L. Fantini,
M. Faria,
K. Farmer,
F. Fassin,
D. Fazzini,
L. Felkowski,
C. Feng,
M. Feng,
A. Fernandez Casani,
M. Fernandez Gomez,
B. Fernandez Rodino,
J. Fernandez-John,
A.D. Fernez,
F. Ferrari,
F. Ferreira Rodrigues,
R.A. Fini,
R. Fiorenza,
M. Fiorini,
M. Firlej,
D.S. Fitzgerald,
C. Fitzpatrick,
T. Fiutowski,
F. Fleuret,
A. Fomin,
M. Fontana,
M. Fontes Vaz,
L.A. Foreman,
R. Forty,
D. Foulds-Holt,
V. Franco Lima,
M. Franco Sevilla,
M. Frank,
E. Franzoso,
G. Frau,
C. Frei,
D.A. Friday,
M. Fritsch,
J. Fu,
Y. Fu,
Q. F\"uhring,
T. Fulghesu,
M. Fulghieri,
M.D. Galati,
A. Gallas Torreira,
D. Galli,
S. Gambetta,
M. Gandelman,
P. Gandini,
B. Ganie,
H. Gao,
R. Gao,
T.Q. Gao,
Y. Gao,
Y. Gao,
Y. Gao,
L.M. Garcia Martin,
P. Garcia Moreno,
B. Gardinovacki,
P. Gardner,
L. Garrido,
C. Gaspar,
A. Gavrikov,
J. George,
E. Gersabeck,
M. Gersabeck,
T. Gershon,
S. Ghizzo,
Z. Ghorbanimoghaddam,
F.I. Giasemis,
V. Gibson,
H.K. Giemza,
A.L. Gilman,
M. Giovannetti,
A. Giovent\`u,
L. Girardey,
M.A. Giza,
F.C. Glaser,
V.V. Gligorov,
C. G\"obel,
L. Golinka-Bezshyyko,
E. Golobardes,
A. Golutvin,
S. Gomez Fernandez,
A.G. Gomez Mongui,
W. Gomulka,
F. Goncalves Abrantes,
I. Gon\c{c}ales Vaz,
M. Goncerz,
G. Gong,
S. Gong,
J.A. Gooding,
C. Gotti,
E. Govorkova,
J.P. Grabowski,
L.A. Granado Cardoso,
R. Grande Quartieri,
E. Graug\'es,
E. Graverini,
L. Grazette,
G. Graziani,
A.T. Grecu,
N.A. Grieser,
L. Grillo,
C. Gu,
M. Guarise,
L. Guerry,
M. Guittiere,
A.-K. Guseinov,
Y. Guz,
T. Gys,
K. Habermann,
T. Hadavizadeh,
C. Hadjivasiliou,
G. Haefeli,
C. Haen,
S. Haken,
G. Hallett,
P.M. Hamilton,
Q. Han,
S. Han,
X. Han,
S. Hannon,
S. Hansmann-Menzemer,
N. Harnew,
T.J. Harris,
L. Hartman,
M. Hartmann,
S. Hashmi,
J. He,
N. Heatley,
A. Hedes,
F. Hemmer,
C. Henderson,
R. Henderson,
R.D.L. Henderson,
A.M. Hennequin,
K. Hennessy,
A. Henrot,
J. Herd,
P. Herrero Gascon,
J. Heuel,
A. Heyn,
A. Hicheur,
G. Hijano Mendizabal,
J.N. Himbert,
P. Hoffmann,
J. Horswill,
R. Hou,
Y. Hou,
D.C. Houston,
N. Howarth,
W. Hu,
X. Hu,
W. Hulsbergen,
R.J. Hunter,
D. Hutchcroft,
M. Idzik,
P. Ilten,
A. Iohner,
S. Jacevicius,
H. Jage,
S.J. Jaimes Elles,
S. Jakobsen,
T. Jakoubek,
E. Jans,
A. Jawahery,
C. Jayaweera,
A. Jelavic,
V. Jevtic,
Z. Jia,
E. Jiang,
X. Jiang,
Y. Jiang,
Y.J. Jiang,
E. Jimenez Moya,
N. Jindal,
M. John,
A. John Rubesh Rajan,
D. Johnson,
C.R. Jones,
S. Joshi,
B. Jost,
J. Juan Castella,
N. Jurik,
I. Juszczak,
D. Kaminaris,
S. Kandybei,
M. Kane,
Y. Kang,
C. Kar,
A. Kauniskangas,
J.W. Kautz,
M.K. Kazanecki,
F. Keizer,
M. Kenzie,
T. Ketel,
B. Khanji,
S. Kholodenko,
V. Kholoimov,
G. Khreich,
Y. Khyzhniak,
F. Kiraz,
T. Kirn,
V.S. Kirsebom,
N. Kleijne,
A. Kleimenova,
D. Klekots,
K. Klimaszewski,
M.R. Kmiec,
T. Knospe,
R. Kolb,
S. Koliiev,
L. Kolk,
A. Konoplyannikov,
P. Kooij,
P. Kopciewicz,
P. Koppenburg,
A. Korchin,
D. Kosianov,
I. Kostiuk,
O. Kot,
S. Kotriakhova,
E. Kowalczyk,
O. Kravcov,
M. Kreps,
W. Krupa,
W. Krzemien,
O. Kshyvanskyi,
S. Kubis,
M. Kucharczyk,
A. Kupsc,
A. Kurzina,
V. Kushnir,
B. Kutsenko,
I. Kyryllin,
D. Lacarrere,
P. Laguarta Gonzalez,
A. Lai,
A. Lampis,
D. Lancierini,
C. Landesa Gomez,
G. Lanfranchi,
C. Langenbruch,
T. Latham,
F. Lazzari,
R. Le Gac,
B. Leban,
H. Lee,
R. Lef\`evre,
M. Lehuraux,
C. Lemettais,
E. Lemos Cid,
O. Leroy,
T. Lesiak,
E.D. Lesser,
B. Leverington,
A. Li,
C. Li,
C. Li,
H. Li,
J. Li,
K. Li,
L. Li,
L. Li,
P. Li,
P.-R. Li,
Q. Li,
T. Li,
T. Li,
W. Li,
Y. Li,
Y. Li,
Y. Li,
Z. Li,
Z. Lian,
Q. Liang,
X. Liang,
Z. Liang,
S. Libralon,
A. Lightbody,
J. Lin,
S. Lin,
T. Lin,
R. Lindner,
H. Linton,
R. Litvinov,
D. Liu,
F.L. Liu,
G. Liu,
K. Liu,
S. Liu,
W. Liu,
X. Liu,
Y. Liu,
Y. Liu,
Y.L. Liu,
G. Loachamin Ordonez,
I. Lobo,
A. Lobo Salvia,
A. Loi,
T. Long,
D. Loomis,
F.C.L. Lopes,
J.H. Lopes,
B. Lopes Pereira,
A. Lopez Huertas,
C. Lopez Iribarnegaray,
A. Lozar,
Q. Lu,
S. Lu,
Y. Lu,
C. Lucarelli,
D. Lucchesi,
M. Lucio Martinez,
A. Lupato,
M. Lupberger,
E. Luppi,
K. Lynch,
J. Lyu,
S. Lyu,
X.-R. Lyu,
H. Ma,
S. Maccolini,
F. Machefert,
F. Maciuc,
B. Mack,
I. Mackay,
L.M. Mackey,
L.R. Madhan Mohan,
M.J. Madurai,
D. Magdalinski,
B. Maisano,
J.J. Malczewski,
S. Malde,
L. Malentacca,
G. Manca,
A. Mangalasseri,
F. Manganella,
R. Mangrulkar,
A. Manoj Nair,
D. Manuzzi,
S. Mao,
D. Marangotto,
J.F. Marchand,
R. Marchevski,
U. Marconi,
L. Mareso,
E. Mariani,
S. Mariani,
C. Marin Benito,
J. Marks,
A.M. Marshall,
L. Martel,
G. Martelli,
L. Martinazzoli,
M. Martinelli,
C. Martinez,
A. Martinez Armas,
D. Martinez Gomez,
D. Martinez Santos,
F. Martinez Vidal,
A. Martorell i Granollers,
A. Massafferri,
R. Matev,
A. Mathad,
C. Matteuzzi,
K.R. Mattioli,
L. Matzner,
A. Mauri,
E. Maurice,
J. Mauricio,
P. Mayencourt,
J. Mazorra de Cos,
M. Mazurek,
D. Mazzanti Tarancon,
M. McCann,
N.T. McHugh,
A. McNab,
R. McNulty,
S.E.R. Medaer,
D. Melnychuk,
D. Mendoza Granada,
P. Menendez Valdes Perez,
F.M. Meng,
M. Merk,
A. Merli,
L. Meyer Garcia,
D. Miao,
H. Miao,
S. Mico,
M. Mikhasenko,
D.A. Milanes,
A. Minotti,
E. Minucci,
B. Mitreska,
D.S. Mitzel,
R. Mocanu,
A. Modak,
L. Moeser,
R.D. Moise,
E.F. Molina Cardenas,
T. Momb\"acher,
M. Monk,
T. Monnard,
S. Monteil,
A. Morcillo Gomez,
G. Morello,
M.J. Morello,
M.P. Morgenthaler,
A. Moro,
J. Moron,
W. Morren,
A.B. Morris,
A.G. Morris,
R. Mountain,
Z. Mu,
N. Muangkod,
E. Muhammad,
F. Muheim,
M. Mulder,
K. M\"uller,
M. Myers,
V. Mytrochenko,
P. Naik,
T. Nakada,
G. Napoletano,
I. Nasteva,
M. Needham,
N. Neri,
S. Neubert,
N. Neufeld,
J. Nicolini,
D. Nicotra,
E.M. Niel,
L. Nisi,
Q. Niu,
B.K. Njoki,
P. Nogarolli,
P. Nogga,
J. Nombela Royo,
E. Noomen,
C. Normand,
A. Novo Cal,
J. Novoa Fernandez,
G. Nowak,
H.N. Nur,
A. Oblakowska-Mucha,
T. Oeser,
T. Ogasa,
O. Okhrimenko,
R. Oldeman,
N. Oldman,
F. Oliva,
E. Olivart Pino,
M. Olocco,
M. Omana Kuttan,
R.H. O'Neil,
J.S. Ordonez Soto,
D. Osthues,
J.M. Otalora Goicochea,
A. Oyanguren,
O. Ozcelik,
F. Paciolla,
A. Padee,
K.O. Padeken,
B. Pagare,
T. Pajero,
A. Palano,
L. Palini,
L. Palombini,
M. Palutan,
C. Pan,
X. Pan,
S. Panebianco,
S. Paniskaki,
L. Paolucci,
A. Papanestis,
M. Pappagallo,
L.L. Pappalardo,
C. Pappenheimer,
C. Parkes,
D. Parmar,
A. Parry,
G. Passaleva,
D. Passaro,
A. Pastore,
M. Patel,
J. Patoc,
C. Patrignani,
A. Paul,
C.J. Pawley,
A. Pellegrino,
J. Peng,
X. Peng,
M. Pepe Altarelli,
S. Perazzini,
M. Pereira Martinez,
C. Perez,
A. Perez Casas,
P. Perret,
A. Perrevoort,
A. Perro,
R. Pestotnik,
M.J. Peters,
A. Petkovic,
K. Petridis,
A. Petrolini,
S. Pezzulo,
J.P. Pfaller,
H. Pham,
L. Pica,
E. Picatoste Olloqui,
M. Piccini,
L. Piccolo,
F. Piernas Diaz,
B. Pietrzyk,
R.N. Pilato,
D. Pinci,
F. Pisani,
M. Pizzichemi,
V.M. Placinta,
M. Plo Casasus,
T. Poeschl,
F. Polci,
M. Poli Lener,
A. Poluektov,
I. Polyakov,
E. Polycarpo,
S. Ponce,
D. Popov,
K. Popp,
K. Prasanth,
C. Prouve,
D. Provenzano,
P. Prus,
V. Pugatch,
A. Puicercus Gomez,
G. Punzi,
J.R. Pybus,
M.P. Pycior,
Q. Qian,
W. Qian,
N. Qin,
R. Quagliani,
R.I. Rabadan Trejo,
B. Rachwal,
R. Racz,
J.H. Rademacker,
M. Rama,
M. Ram\'irez Garc\'ia,
M. Ramirez Trujillo,
V. Ramos De Oliveira,
M. Ramos Pernas,
G. Ramsey,
M.S. Rangel,
G. Raven,
M. Rebollo De Miguel,
F. Redi,
J. Reich,
F. Reiss,
Z. Ren,
M. Ribalda Galvez,
R. Ribatti,
G. Ricart,
D. Riccardi,
S. Ricciardi,
K. Richardson,
M. Richardson-Slipper,
F. Riehn,
K. Rinnert,
P. Robbe,
G. Robertson,
E. Rodrigues,
A. Rodriguez Alvarez,
E. Rodriguez Fernandez,
J.A. Rodriguez Lopez,
E. Rodriguez Rodriguez,
J. Roensch,
A. Rogovskiy,
D.L. Rolf,
P. Roloff,
A. Romano,
V. Romanovskiy,
A. Romero Vidal,
G. Romolini,
F. Ronchetti,
T. Rong,
W. Rose,
M. Rotondo,
M.S. Rudolph,
G. Ruggiero,
M. Ruiz Diaz,
J. Ruiz Vidal,
J. Ruz Armendariz,
J.J. Saavedra-Arias,
J.J. Saborido Silva,
D. Sahoo,
N. Sahoo,
B. Saitta,
M. Salomoni,
I. Sanderswood,
R. Santacesaria,
C. Santamarina Rios,
M. Santimaria,
L. Santoro ,
E. Santovetti,
A. Saputi,
A. Sarnatskiy,
G. Sarpis,
M. Sarpis,
A. Satta,
M. Saur,
H. Sazak,
F. Sborzacchi,
A. Scarabotto,
S. Schael,
S. Scherl,
M. Schiller,
H. Schindler,
M. Schmelling,
B. Schmidt,
N. Schmidt,
S. Schmitt,
H. Schmitz,
O. Schneider,
A. Schopper,
N. Schulte,
H. Schumacher,
M.H. Schune,
G. Schwering,
B. Sciascia,
A. Sciuccati,
G. Scriven,
I. Segal,
A. Seljak,
S. Sellam,
M. Senghi Soares,
A. Sergi,
N. Serra,
L. Sestini,
B. Sevilla Sanjuan,
D.M. Shangase,
R. Sharma,
L. Shchutska,
T. Shears,
S. Shelton,
J. Shen,
Z. Shen,
S. Sheng,
B. Shi,
J. Shi,
Q. Shi,
W.S. Shi,
E. Shmanin,
O. Sidletskiy,
R. Silva Coutinho,
G. Simi,
S. Simone,
M. Singha,
I. Siral,
N. Skidmore,
T. Skwarnicki,
M.W. Slater,
E. Smith,
M. Smith,
M. Smith,
L. Soares Lavra,
M.D. Sokoloff,
F.J.P. Soler,
A. Solomin,
K. Solovieva,
N.S. Sommerfeld,
R. Song,
Y. Song,
Y. Song,
Y.S. Song,
F.L. Souza De Almeida,
G. Souza De Castro,
B. Souza De Paula,
K.M. Sowa,
E. Spadaro Norella,
J.G. Speer,
P. Spradlin,
F. Stagni,
M. Stahl,
S. Stahl,
S. Stanislaus,
O. Steinkamp,
F. Suljik,
J. Sun,
L. Sun,
M. Sun,
P. Svihra,
V. Svintozelskyi,
J. Swallow,
K. Swientek,
F. Swystun,
A. Szabelski,
T. Szumlak,
Y. Tan,
Y. Tang,
Y.T. Tang,
M. Tariq,
M.D. Tat,
K.L. Taylor,
J.A. Teijeiro Jimenez,
F. Terzuoli,
F. Teubert,
E. Thomas,
D.J.D. Thompson,
A.R. Thomson-Strong,
R. Thornton,
H. Tilquin,
V. Tisserand,
S. T'Jampens,
M. Tobin,
T.T. Todorov,
L. Tomassetti,
G. Tonani,
X. Tong,
T. Tork,
L. Torlai,
L. Toscano,
D.Y. Tou,
T. Troska,
G. Tuci,
N. Tuning,
L.H. Uecker,
A. Ukleja,
A. Upadhyay,
B. Urbach,
A. Usachov,
U. Uwer,
V. Vagnoni,
A. Vaitkevicius,
A. Valassi,
V. Valcarce Cadenas,
G. Valenti,
N. Valls Canudas,
J. van Eldik,
H. Van Hecke,
E. van Herwijnen,
C.B. Van Hulse,
R. Van Laak,
M. van Veghel,
P. Varrella,
R. Vazquez Gomez,
P. Vazquez Regueiro,
C. V\'azquez Sierra,
S. Vecchi,
J. Velilla Serna,
J.J. Velthuis,
M. Veltri,
A. Venkateswaran,
M. Verdoglia,
M. Vesterinen,
W. Vetens,
D. Vico Benet,
P. Vidrier Villalba,
M. Vieites Diaz,
X. Vilasis-Cardona,
E. Vilella Figueras,
A. Villa,
P. Vincent,
B. Vivacqua,
F.C. Volle,
D. vom Bruch,
K. Vos,
C. Vrahas,
J. Wagner,
J. Walsh,
N. Walter,
E.J. Walton,
G. Wan,
A. Wang,
B. Wang,
C. Wang,
C. Wang,
C. Wang,
G. Wang,
H. Wang,
J. Wang,
J. Wang,
J. Wang,
J. Wang,
M. Wang,
N.W. Wang,
X. Wang,
X. Wang,
X.W. Wang,
Y. Wang,
Y. Wang,
Y. Wang,
Y.H. Wang,
Z. Wang,
Z. Wang,
M. Waterlaat,
N.K. Watson,
D. Websdale,
Y. Wei,
Z. Weida,
J. Wendel,
B.D.C. Westhenry,
A.S. White,
C. White,
M. Whitehead,
E. Whiter,
A.R. Wiederhold,
D. Wiedner,
M.A. Wiegertjes,
C. Wild,
G. Wilkinson,
M.K. Wilkinson,
M. Williams,
M.J. Williams,
M.R.J. Williams,
R. Williams,
S. Williams,
Z. Williams,
F.F. Wilson,
M. Winn,
W. Wislicki,
M. Witek,
L. Witola,
T. Wolf,
E. Wood,
G. Wormser,
S.A. Wotton,
H. Wu,
J. Wu,
T. Wu,
X. Wu,
Y. Wu,
Z. Wu,
K. Wyllie,
S. Xian,
Z. Xiang,
Y. Xie,
T.X. Xing,
A. Xu,
L. Xu,
M. Xu,
R. Xu,
Z. Xu,
Z. Xu,
Z. Xu,
Z. Xu,
S. Yadav,
K. Yang,
X. Yang,
Y. Yang,
Y. Yang,
Z. Yang,
Z. Yang,
H. Yeung,
H. Yin,
X. Yin,
C.Y. Yu,
J. Yu,
K. Yu,
X. Yuan,
Y Yuan,
E. Zaffaroni,
S. Zalambani,
J.A. Zamora Saa,
F. Zangari,
M. Zavertyaev,
M. Zdybal,
F. Zenesini,
C. Zeng,
M. Zeng,
S.H Zeng,
C. Zhang,
C. Zhang,
D. Zhang,
J. Zhang,
L. Zhang,
Q.Z. Zhang,
R. Zhang,
S. Zhang,
S.L. Zhang,
Y. Zhang,
Z. Zhang,
J. Zhao,
M. Zhao,
Y. Zhao,
A. Zhelezov,
S.Z. Zheng,
X.Z. Zheng,
Y. Zheng,
T. Zhou,
X. Zhou,
V. Zhovkovska,
L.Z. Zhu,
X. Zhu,
X. Zhu,
Y. Zhu,
V. Zhukov,
J. Zhuo Gao,
T. Zies,
D. Zuliani,
X. Zuo
